Federated Learning via Decentralized Dataset Distillation in Resource-Constrained Edge Environments

In federated learning, all networked clients contribute to the model training cooperatively. However, with model sizes increasing, even sharing the trained partial models often leads to severe communication bottlenecks in underlying networks, especially when communicated iteratively. In this paper, we introduce a federated learning framework FedD3 requiring only one-shot communication by integrating dataset distillation instances. Instead of sharing model updates in other federated learning approaches, FedD3 allows the connected clients to distill the local datasets independently, and then aggregates those decentralized distilled datasets (e.g. a few unrecognizable images) from networks for model training. Our experimental results show that FedD3 significantly outperforms other federated learning frameworks in terms of needed communication volumes, while it provides the additional benefit to be able to balance the trade-off between accuracy and communication cost, depending on usage scenario or target dataset. For instance, for training an AlexNet model on CIFAR-10 with 10 clients under non-independent and identically distributed (Non-IID) setting, FedD3 can either increase the accuracy by over 71% with a similar communication volume, or save 98% of communication volume, while reaching the same accuracy, compared to other one-shot federated learning approaches.

==> appendices/A_notations.tex <==
\section{Abbreviations and Notations}
\label{subsec:A}

We provide overviews of the most relevant notations and abbreviations in Tab.~\ref{table:notation} and Tab.~\ref{table:abbreviation}, respectively.

\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}



\begin{table*}[ht!]
\centering
\begin{threeparttable}
\caption{\centering Summary of mainly used notations in this paper.}
\label{table:notation}
\begin{tabular}{M{1.5cm}L{10.9cm}M{2cm}}
   \toprule %%%%%%%%%%%%%%%%%%
    \centering\textbf{Notation} & \centering\textbf{Meaning}  & \textbf{Navigation}\\
    \midrule %%%%%%%%%%%%%%%%%%

    $m$  & Number of clients in federated learning systems, $m \in \mathbb{N}_+$ & Sec.~3 \\

    $k$  & Index of a set of clients,  $k \in \mathbb{N}_+, 1 \leq k \leq m $  & Sec.~3\\
    
    $\mathcal{D}$ & Global dataset, see Eq.~\ref{Eq:D} & Sec.~3\\
    
    $\mathcal{D}_k$ & Local dataset in the client $k$, see Eq.~\ref{Eq:D_k} & Sec.~3\\
     
    $\mathcal{\tilde D}$ & Aggregated distilled dataset in the server, see Eq.~\ref{Eq:D_d} & Sec.~3\\
    
    $\mathcal{\tilde D}_k$ &  Distilled dataset in local dataset in the client $k$, see Eq.~\ref{Eq:D_kd} & Sec.~3\\

    $n$  & Number of data points in global dataset, $n=|\mathcal{D}_k|$ & Sec.~3 \\
    
    $n_k$  & Number of data points in local dataset in the client $k$, $n=|\mathcal{D}|$ & Sec.~3 \\
    
    $\tilde n$  & Number of aggregated distilled data points in the server, $n=|\mathcal{\tilde D}|$ & Sec.~3 \\
    
    $\tilde n_k$  & Number of distilled data points from the client $k$, $n=|\mathcal{\tilde D}_k|$ & Sec.~3 \\

    $i$, $j$  & Index of data points & Sec.~3 \\
    
    $s$  & Index of class of labeled data points & Sec.~3 \\
    
    $S$  & A set of classes of a labeled dataset, $s\in S$ & Sec.~3 \\
    
    $S_k$  & A set of classes of a labeled local dataset in the client $k$, $S_k\subseteq S$ & Sec.~3 \\

    $C_k$  & Number of classes in client $k$, $C_k = |S_k|$ & Sec.~3 \\
    
    $X$  & Matrix of stacked data points $x$, see Eq.~\ref{Eq:X} & Sec.~3 \\
    
    $X_k$  &  Matrix of stacked data points $x_k$, see Eq.~\ref{Eq:X_k} & Sec.~3 \\
    
    $\tilde X$  &  Matrix of stacked data points $\tilde x$, see Eq.~\ref{Eq:X_d} & Sec.~3 \\
    
    $\tilde X_k$  &  Matrix of stacked data points $\tilde x_k$, see Eq.~\ref{Eq:X_kd} & Sec.~3 \\

    $y_i$ & The label of the data point $i$ & Sec.~3\\
    
    $y_k$ & The label vector in the client $k$  & Sec.~3\\

    $\Theta$ & Hyper-parameters in kernel function  & Sec.~3\\
    
    $\Theta_k$ & Hyper-parameters in kernel function  & Sec.~3\\

    $e$ & Index of epochs   & Sec.~3\\

    $E$ & Index of the global training epochs  & Sec.~3\\

    $e_k$ & Index of the local distilling (training) epochs & Sec.~3\\

    $E_k$ & Number of the local distilling (training) epochs & Sec.~3\\
    
    $b$ & Index of batches & Sec.~3\\
    
    $X_b$ & Matrix of stacked data points in the batch $b$ & Sec.~3\\
    
    $y_b$ &  Label vector of the batch $b$ & Sec.~3\\

    $\mathcal{\tilde B}_k$ &  Batch set of synthetic data points for the distilling in the client $k$  & Sec.~3\\
    
    $\mathcal{\tilde B}$ & Batch set of aggregated distilled data points for the training in the server & Sec.~3\\
    
    $t$ &  Index of the communication rounds  & Sec.~3\\
    
    $T$ & Number of the communication rounds  & Sec.~3\\
    
%    $K_k$ &  Kernel function of KIP-based instance in the local client $k$ & Sec.~3\\
    
    $\eta$ & Global learning rate  & Sec.~3\\
    
    $\eta_k$ & Local learning rate in the client $k$ & Sec.~3\\
    
    $V_t$ & Communication volume (bit) in the communication round $t$ & Sec.~3\\
    
    $P$ & Bit size of models & Sec.~4\\
    

    

    \bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table*}
\newcommand{\vecline}{~~~\rule[.5ex]{2em}{0.4pt}~~~}

\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
    \label{Eq:D}
    \mathcal{D} = \{x_i|i=1,2,...,n \}
\end{equation}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
    \label{Eq:D_k}
    \mathcal{D}_k = \{x_{k,i}|i=1,2,...,n_k \}
\end{equation}
\end{minipage}

\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
    \label{Eq:D_d}
    \mathcal{\tilde D} = \{\tilde x_{j}|j=1,2,...,\tilde n \}
\end{equation}

\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\begin{equation}
    \label{Eq:D_kd}
    \mathcal{\tilde D}_k = \{\tilde x_{k,j}|j=1,2,...,\tilde n_k \}
\end{equation}
\end{minipage}











\begin{minipage}[t]{0.5\textwidth}

\begin{equation}
    \label{Eq:X}
    X = 
  \begin{bmatrix}
  \vecline x_{1} \vecline \\
  \vdots \\
  \vecline x_{i} \vecline \\
  \vdots\\
  \vecline x_{n} \vecline \\
  \end{bmatrix}
\end{equation}

\end{minipage}
\begin{minipage}[t]{0.5\textwidth}

\begin{equation}
    \label{Eq:X_k}
    X_k = 
  \begin{bmatrix}
  \vecline x_{k,1} \vecline \\
  \vdots \\
  \vecline x_{k,i} \vecline \\
  \vdots\\
  \vecline x_{k,n} \vecline \\
  \end{bmatrix}
\end{equation}

\end{minipage}

\begin{minipage}[t]{0.5\textwidth}

\begin{equation}
    \label{Eq:X_d}
    \tilde X = 
  \begin{bmatrix}
  \vecline \tilde x_{1} \vecline \\
  \vdots \\
  \vecline \tilde x_{j} \vecline \\
  \vdots\\
  \vecline \tilde x_{n} \vecline \\
  \end{bmatrix}
\end{equation}

\end{minipage}
\begin{minipage}[t]{0.5\textwidth}

\begin{equation}
    \label{Eq:X_kd}
    \tilde X_k = 
  \begin{bmatrix}
  \vecline \tilde x_{k,1} \vecline \\
  \vdots \\
  \vecline \tilde x_{k,j} \vecline \\
  \vdots\\
  \vecline \tilde x_{k,n} \vecline \\
  \end{bmatrix}
\end{equation}

\end{minipage}




\begin{table*}[ht!]
\centering
\begin{threeparttable}
\caption{\centering Summary of mainly used abbreviations in this paper.}
\label{table:abbreviation}
\begin{tabular}{M{1.8cm}L{10.7cm}M{2cm}}
   \toprule %%%%%%%%%%%%%%%%%%
    \centering\textbf{Abbr.} & \centering\textbf{Meaning}  & \textbf{Navigation}\\
    \midrule %%%%%%%%%%%%%%%%%%
    
    (Non-) IID &  (Non-) Independent and Identically Distributed & Sec.~1\\
        
    FedD3 &  Federated Learning from Decentralized Distilled Datasets (Our framework) & Sec.~1\\
    
    ACC &  Prediction Accuracy & Sec.~3\\
    
    \myECEAbbr &  \myECEFull ($\gamma$-\myECEAbbr indicates \myECEAbbr at specific $\gamma$) & Sec.~3\\
    
    DD &  Dataset Distillation  & Sec.~3\\
    
    Img/Cls & Contributed number of distilled images per class from one client  & Sec.~4\\
    
%    KIP &  Kernel Inducing Points & Sec.~\ref{sec:intro}\\
    
    OSFL & One-Shot Federated Learning  & Sec.~4\\
     
    MSFL & Multi-Shot Federated Learning  & Sec.~4\\
    
%    D2D &  Device to Device & Sec.5\\
    
%    D2N &  Device to Networks & Sec.5\\

    %
    \bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\end{threeparttable}
\end{table*}




==> appendices/B_futher_datasets.tex <==
\section{Datasets}
\label{subsec:B}

\setcounter{table}{0}
\renewcommand{\thetable}{B\arabic{table}}

We visualize the distilled images from Fashion-MNIST~\citep{xiao2017/online} in different distillation steps in Fig.~\ref{fig:dd_FashionMnist}.
%
In Fig.~\ref{fig:further_datasets_vis}, we further visualize the distilled images from decentralized distilled Fashion-MNIST and SVHN, where pathological Non-IID~\citep{huang2021personalized} datasets are distributed in 10 clients. We use five datasets totally for the experiments:
\begin{itemize}
    \item CIFAR-10~\citep{cifar10}: 50000 data points in the training set and 10000 data points in the test set. Each data point is a 32x32 RGB image, associated with a label from 10 classes
    \item Fashion-MNIST~\citep{xiao2017/online}: 60000 data points in the training set and 10000 data points in the test set. Each data point is a 28x28 gray-scale image, associated with a label from 10 classes
    \item MNIST~\citep{mnist-2010}: 60000 data points in the training set and 10000 data points in the test set. Each data point is a 28x28 gray-scale digit image, associated with a label from 10 classes
    \item SVHN~\citep{netzer2011reading}: 73257 data points in the training set and 26032 data points in the test set. Each data point is a 32x32 RGB digit image, associated with a label from 10 classes
    \item CIFAR-100~\citep{netzer2011reading}: 50000 data points in the training set and 10000 data points in the test set. Each data point is a 32x32 RGB image, associated with a label from 100 classes.
\end{itemize}

\setcounter{figure}{0}                       
\renewcommand\thefigure{B.\arabic{figure}}   

\begin{figure*}[h!]
\centering
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/dd_FashionMnist.PNG}
\caption{Visualization of dataset distillation on IID Fashion-MNIST datasets for 10 classes with increasing distillation steps}
\label{fig:dd_FashionMnist}
\end{figure*}


\begin{figure*}[h!]
\centering
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/ResVis_furtherDatasets_v2.png}
\caption{Decentralized distilled datasets from 10 clients. The Fashion-MNIST and SVHN datasets are respectively distributed in 10 clients. The local dataset in each client consists of only two classes.}
\label{fig:further_datasets_vis}
\end{figure*}



==> appendices/C_hyperparameters.tex <==
\section{Details on Experiments}
\label{subsec:C}

In this section, we report details on datasets, federated system parameters, and hyperparameters in our framework as well as in baselines in our experiments in Sec.~4.3, which run on a computer cluster with 4$\times$~NVIDIA-A100-PCIE-40GB GPUs and 4$\times$~32-Core-AMD-EPYC-7513 CPUs. The environment is a Linux system with Pytorch 1.8.1 and Cuda 11.1.

%
We divide the datasets (MNIST and CIFAR-10) into 500 clients for model training in federated fashion. 
%
Considering data heterogeneity across clients, we demonstrate \myFedDD and other baselines on both IID and pathological non-IID~\citep{huang2021personalized} datasets. 
%
The number of the data points for each class in each client is almost the same, i.e. the data load for 500 clients is nearly balanced. 
%
For a fair comparison, we do not use any data augmentation methods in \myFedDD and other baselines.
%

%%
We do not consider any compression methods to enhance the \myECEFull (GCE) equally for \myFedDD and baselines, as it is not the focus of this paper.
%
In fact, as mentioned in the paper, the standard federated learning (except on-shot federated learning) methods still require communication cost for downloading the global models.
%
Also, as the type of parameters in images can be uint8 and in models can be float32 or float16 (half precision), the messages for distilled datasets can be compressed smaller.

We compare \myFedDD with eight baselines, four federated learning methods in both one-shot and multi-shot federated fashions. The four methods and the associated parameters are followed: 
(\emph{i}) FedAvg~\citep{pmlr-v54-mcmahan17a}; (\emph{ii}) FedProx~\citep{li2020federated} ($\mu=0.1$); (\emph{iii}) FedNova~\citep{wang2020tackling}; (\emph{iv}) SCAFFOLD~\citep{SCAFFOLD}.
%


For MSFL, each client trains models on local dataset with fixing 10 epochs between every two communication rounds. 
%
We use stochastic gradient descent (SGD) with fixing learning rate from $\{0.001, 0.025\}$, momentum 0.9, batch size 50 and number of local epochs from $\{10, 50\}$. 
%
Note that we use the same learning rate in \myFedDD and baselines for a fair comparison.
%
we let each test run 10 times with 10 different seeds and use the mean value as the evaluation results.
%
Considering the communication cost explodes with the increasing communication rounds, only the first 18 and 6 communication rounds for the training on MNIST and CIFAR-10 are considered for the evaluation, respectively, otherwise \myECEAbbr reduces rapidly, due to the increasing of the total communication volume.

For OSFL, the number of local epochs before the one-shot communication matters~\citep{pmlr-v54-mcmahan17a, li2022federated}. The federated learning with more local epochs can train the model more fully in clients, however can lead to overfitting on local datasets. Thus, we set the number of local epochs from $\{1, 10, 50, 100, 150\}$ on MNIST and from $\{1, 5, 10, 20, 50\}$ on CIFAR-10 for all methods.
%
Specifically for Non-IID MNIST, we have observed the pure one-shot can not achieve good results, as shown in Fig.~2.
%\ref{fig:acc-msg}. 
%
Thus, we run one pre-aggregation for all clients before the OSFL for a much better evaluation results in baselines. 
%
Each method runs with each of those values 5 times with different seeds.
%
Finally, only the best 5 results out of 25 tests are considered for the evaluation.

For \myFedDD, we integrate both coreset- and KIP-based instances. We let each client distill only 1 synthetic image per class and upload them to server, i.e. each client contributes 2 distilled images on Non-IID dataset and 10 distilled images on IID dataset.
%
That also explains why \myFedDD may achieve a better test accuracy but with lower \myECEAbbr on IID dataset than on Non-IID dataset.
%
Specifically, we use Gaussian mixture model to perform the \myFedDD with coreset-based instance.
%
For KIP-based instance, we use a 4-layer and 1024-width fully connected model distill the dataset with distillation learning rate 0.004 and batch size 10\% of local dataset size. 
%
We set a maximum number of epochs on 3000 and a threshold of distillation accuracy on 0.999.
%
If the threshold is exceeded, the distillation loop breaks out immediately and the client is ready to upload the synthetic images.

%%
Beside the comparison results on MNIST and CIFAR-10 in Tab.3, we further conduct the experiments for training a ResNet-18~\citep{he2016deep} on Fashion-MNIST and SVHN, and training a CNN on CIFAR-100 using MSFL, OSFL and \myFedDD in Tab.4.
%
Note that for MSFL, We select the best result in the first 3, 9 and 15 communication rounds for the training on Fashion-MNIST, SVHN and CIFAR-100, respectively.
%
The best results among their corresponding instances are shown in Tab.~3. 
%
Note that the Img/Cls for the tests on SVHN is 10, other hyperparameters are the same as in Tab.~2.

%%
As we expected, on IID datasets, \myFedDD can achieve comparable test prediction accuracy with much better \myECEAbbr. 
%
On Non-IID datasets, \myFedDD outperforms both MSFL and OSFL in terms of accuracy and communication efficiency. 
%
The two biggest advantages of \myFedDD, i.e. communication efficiency and robustness to data heterogeneity, are experimentally validated, which is consistent with the conclusions in Tab.~2.


==> appendices/D_further_comparsion.tex <==
\section{Comparison on Further Datasets}
\label{subsec:D}

%%
Beside the comparison results on MNIST and CIFAR-10 in Tab.~\ref{table:comparison}, we further conduct the experiments for training a ResNet-18~\citep{he2016deep} using MSFL, OSFL and \myFedDD on Fashion-MNIST and SVHN. 
%
Note that for MSFL, We select the best result in the first 3 and 9 communication rounds for the training on Fashion-MNIST and SVHN, respectively.
%
The best results among their corresponding instances are shown in Tab.~\ref{table:benchmark_further}. 
%
Note that the Img/Cls for the tests on SVHN is 10, other hyperparameters are the same as in Tab.~\ref{table:comparison}.

%%
As we expected, on IID datasets, \myFedDD can achieve comparable test prediction accuracy with much better \myECEAbbr. 
%
On Non-IID datasets, \myFedDD outperforms both MSFL and OSFL in terms of accuracy and communication efficiency. 
%
The two biggest advantages of \myFedDD, i.e. communication efficiency and robustness to data heterogeneity, are experimentally validated, which is consistent with the conclusions in Tab.~\ref{table:comparison}.



\setcounter{table}{0}
\renewcommand{\thetable}{D\arabic{table}}
\input{appendices/D_1_table_further_comparison}




==> appendices/E_further_models.tex <==
\section{Evaluation with Further Models}
\label{subsec:E}

\setcounter{figure}{0}                       
\renewcommand\thefigure{D.\arabic{figure}}

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/Further_Model_v2.png}
\caption{Evaluation for OSFL with further model sizes}
\label{fig:ResNet}
\end{wrapfigure}

In this paper, LeNet and AlexNet are mainly used for evaluation, as both of them are compact and can achieve good test accuracy on MNIST and CIFAR-10, respectively. 
%
Though, the accuracy of one-shot federated learning can still be improved using some large-size models, the required communication volume increases linearly with the size of the model.
%
In this section, we extend the evaluation in Fig.~2 and compare \myFedDD with one-shot FedAvg for training 5 variants of ResNet~\citep{he2016deep} with $E_k$ from $\{1, 10, 50, 100, 150\}$ on MNIST. 

%%
As in Fig~\ref{fig:ResNet} shown, on IID dataset, the results of one-shot FedAvg are comparable to most of \myFedDD results in terms of test accuracy, however, much larger size of messages for transmitting models is required. 
%
On Non-IID dataset, \myFedDD outperforms one-shot FedAvg in terms of communication volume notably, as expected.






  



==> appendices/F_hybrid_fl.tex <==
\section{Multi-shot Communication}
\label{subsec:F}

\setcounter{figure}{0}                       
\renewcommand\thefigure{D.\arabic{figure}}  

\begin{figure*}[ht!]
\includegraphics[trim=0 0 0 0,clip,width=1\linewidth]{figures/HybridFl_v2.png}
\caption{The proposed \emph{hybrid federated learning} approach (multi-shot version of \myFedDD) outperforms the standard federated learning on Non-IID decentralized datasets. We consider two local training epoch $E_k$ from $\{1, 5\}$ with batch size $|\mathcal{B}_k|=50$ for each dataset. The Learning rate at $C_k \in \{10, 2\}$ is $0.025$, and at $C_k=1$ is $0.001$.}
\label{fig:hybrid_fl}
\end{figure*}
%%
Due to the robustness on data heterogeneity, we further explore the potential benefits of distilled datasets in federated learning. 
%
We believe that sharing such synthetic data might bridge the information silos. 
%
For that, we extend \myFedDD to multiple shots and consider a hybrid federated learning method by adding a spoon of distilled datasets from other clients via D2N (Device to Networks) or D2D (Device to Device) networks.

In particular, in the first communication round, the client $p$ and receive the global model parameters as well as the distilled datasets in other clients $\mathcal{\tilde D}_p^* = \{\mathcal{\tilde D}_k|k \in \mathbb{N}_+, 1 \leq k \leq m, k \neq p \}$ from the server. Thus, for the client $p$, it trains the model on its local dataset $\mathcal{D}_p$ combing with $\mathcal{\tilde D}_p^*$. 


%We consider \emph{Hybrid Federated Learning} as one federated learning approach, which extends our \myFedDD to multiple communication rounds. As discussed in \emph{A Spoon of Distilled Datasets into Multi-rounds}, we let the decentralized distilled datasets be aggregated at the server before standard federated learning. In the first communication round, the client $p$ and receive the global model parameters as well as the distilled datasets in other clients $\mathcal{\tilde D}_p^* = \{\mathcal{\tilde D}_k|k \in \mathbb{N}_+, 1 \leq k \leq m, k \neq p \}$ from the server. Thus, for the client $p$, it trains the model on its local dataset $\mathcal{D}_p$ combing with $\mathcal{\tilde D}_p^*$. 

We run \emph{hybrid federated learning} to enhance the baseline \emph{FedAvg}~\citep{pmlr-v54-mcmahan17a} and train an AlexNet model on CIFAR-10 distributed in 10 clients with $C_k$ from $\{10, 2, 1\}$. As the evaluation results shown in Fig.~\ref{fig:hybrid_fl}, though, the \emph{hybrid federated learning} can tiny reduce the convergence speed and test accuracy on IID dataset, the \emph{hybrid federated learning} on Non-IID dataset can notably increase the robustness to data heterogeneity. We also notice that even when the \emph{FedAvg} is failed ($E_k=1$ at $C_k=1$), the \emph{hybrid federated learning} can still be convergence in the training.

We believe the distilled datasets from other clients provide each client an insight of global dataset information. Such a multi-shot version of \myFedDD also reveal that dataset distillation technique can provide an effective strategy for improving federated learning performance on Non-IID datasets.




==> appendices/G_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\mypara{Beyond Kernel: Individual DD-instances}
%%
Because of the stable performance, we mainly employ KIP methods as dataset distillation instances in \myFedDD. 
%
In fact, according to the actual local datasets, we can also consider individual instances to generate the synthetic dataset for uploading. 
%
Self-selecting instances in each client should be encouraged, which can be advantageous to the quality of locally distilled datasets, as the server and other clients cannot be not aware of the distribution of local data. 
%
Additionally, we believe the autonomy of local dataset distillation can enhance privacy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mypara{Lessons Learned for Orchestration}
%%
%Our framework allows each client to distill the local dataset, which means all local datasets should meet the requirement of the used dataset distillation method. Here we can think about two example scenarios: 
In \myFedDD, a local dataset should meet the requirement of the used dataset distillation method. Here we can think about two example scenarios: 
%
i) If there is only one data point in one of the clients, $\tilde D_k$ and $D_k$ are the same at the first epoch in \emph{ClientDatasetDistillation} in Algorithm~1;
%
ii) If there is only one data point with its label $x_i$ for a specific class $y_c$, the distilled dataset $\tilde x_i$ can be always the same as $x_i$, especially when only the loss is backpropagated on $\tilde X$. 
%
Both situations can break the privacy, as it will upload at least one raw data point to the server. 
%
To tackle this issue, we believe a good orchestration for dataset and client selection is recommended. 


==> sections/00_abstract_v2.tex <==
\begin{abstract}
In federated learning, a potentially large set of clients contributes to the training of a single final model cooperatively in an iterative process.
%
This is especially attractive in distributed scenarios such as edge or mobile computing applications as data as well as compute capabilities are naturally distributed and this can be used to avoid excessive communication requirements with a central computing resource. 
%
%However, with model sizes increasing, even the sharing of the trained partial models often leads to severe communication bottlenecks in underlying networks, especially when communicated iteratively.
However, with model sizes increasing, even sharing the trained partial models often leads to severe communication bottlenecks in underlying networks, especially when communicated iteratively.
%Rui: I made minor changes here, to avoid half word occupying a single line.
%

In this paper, we introduce a novel federated learning framework, \myFedDD, which reduces the overall communication volume and with that opens up the concept of federated learning to more application scenarios in particular in Bandwidth-constrained networks.
%
This is achieved by leveraging local dataset distillation instead of traditional learning approaches \emph{(i)} to significantly reduce communication volumes and \emph{(ii)} to limit transfers to one-shot communication, rather than relying on iterative multi-way communication.
%
Instead of sharing model updates, as in other federated learning approaches, \myFedDD allows the connected clients to distill the local datasets independently, and then aggregates those decentralized distilled datasets (typically in the form a few unrecognizable images, which are smaller than typical models) across the network only once to form the final model.
%
Our experimental results show that \myFedDD significantly outperforms other federated learning frameworks in terms of needed communication volumes, while it provides the additional benefit to be able to balance the trade-off between accuracy and communication cost, depending on usage scenario or target dataset.
%
%For instance, for an AlexNet model trained on a Non-IID CIFAR-10 dataset ($C_k=5$) distributed in 10 clients,
For instance, for training an AlexNet model on a Non-IID CIFAR-10 dataset ($C_k=5$) with 10 clients,
\myFedDD can either increase the accuracy by over 71\% with a similar communication volume, or save 98\% of communication volume, while reaching the same accuracy, compared to other one-shot federated learning approaches. 
%Moreover, we show that \myFedDD is able to reach the accuracy of other federated learning approaches, while severely limiting the bandwidth that is utilized.
%MS: not sure this helps here - the two points above have impact already
%Moreover, we show that \myFedDD can reach the accuracy of other federated learning approaches, while severely limiting the bandwidth that is utilized.
%Rui: I made minor changes here, to avoid half word occupying a single line. 
%
\end{abstract}



==> sections/06_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Though some previous works in dataset distillation, e.g.~\cite{pmlr-v139-zhao21a}, have mentioned the dataset distillation might be beneficial for federated learning, they have not provided detailed analysis and experimental evaluation on it. 
%

Only little research has explored the dataset distillation approaches in federated learning: Zhou et al.~\cite{zhou2020distilled} 
and Goetz et al.~\cite{goetz2020federated} have attempted to employ the approaches proposed by Wang et al.~\cite{wang2018dataset} and ~\cite{9533769} in federated learning. However, more advanced methods, e.g.~\cite{nguyen2021dataset}~\cite{cazenavette2022distillation} with more stable performance have been developed, and further studies on decentralized dataset distillation in federated settings are needed. Furthermore, both of them have not pointed out the dataset distillation can improve the training on heterogeneous data, which is one of the biggest challenges in federated learning.
%

In fact, the computation abilities in distributed edge devices are normally limited, while most dataset distillation methods require high computation power.  
%
For instance, the approach from Cazenavette
et al.~\cite{cazenavette2022distillation} can lead to computation overhead, though it can generate satisfactory distilled dataset.
%
Therefore, in this work, we consider the coreset-based and KIP-based~\cite{50025, nguyen2021dataset} methods for decentralized dataset distillation in our federated learning framework, and focus on improving the communication efficiency while training on federated datasets.


==> sections/table_presentation.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[!ht]
\centering
\fontsize{7.5}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{The prediction accuracy (ACC) and $\gamma-$\myECEAbbr comparison between \myFedDD and other baselines on both MNIST and CIFAR-10 distributed in 500 clients. %We provide more details on our experiments in the supplementary material.
}
\label{table:comparison}

\begin{tabular}{C{1cm}C{1cm}|C{1.32cm}C{1.32cm}C{1.32cm}C{1.32cm}|C{1.32cm}C{1.32cm}C{1.32cm}C{1.32cm}|C{1.32cm}C{1.32cm}}
\toprule %%%%%%%%%%%%%%%%%%

\multicolumn{2}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{4}{c|}{MSFL\tnote{1}} & \multicolumn{4}{c|}{OSFL} & \multicolumn{2}{c}{FedD3 (Ours)\tnote{2}}\\

&& {FedAvg} & {FedProx} & {FedNova} & {SCAFFOLD} & {FedAvg} & {FedProx} & {FedNova} & {SCAFFOLD} & {Coreset} & {KIP}\\

\midrule %%%%%%%%%%%%%%%%%%
\midrule %%%%%%%%%%%%%%%%%%


\multirow{2}{*}{{MNIST}} & \multirow{1}{*}{ {IID}} & {96.97$\pm$0.02} & {96.55$\pm$0.03} & {85.50$\pm$0.01} & \textbf{97.49$\pm$0.02} & {85.34$\pm$0.02} & {83.63$\pm$0.02} & {74.78$\pm$0.02} & {67.47$\pm$5.89} & {86.82$\pm$0.46} & \textbf{94.37$\pm$0.67}\\

 \cmidrule(lr{0em}){2-12}

& \multirow{1}{*}{ {NIID}} & {71.29$\pm$0.02} & {67.54$\pm$0.04} & {71.33$\pm$0.08} & {88.69$\pm$0.12} & {42.08$\pm$0.03} & {49.25$\pm$0.01} & {63.61$\pm$0.75} & {36.92$\pm$0.03} & {77.29$\pm$2.58} & \textbf{94.74$\pm$0.64}\\

\midrule %%%%%%%%%%%%%%%%%%
\midrule %%%%%%%%%%%%%%%%%%

\multirow{2}{*}{   {CIFAR-10}} & \multirow{1}{*}{ {IID}} & \textbf{48.12$\pm$0.38} & {47.89$\pm$0.27} & {47.69$\pm$0.80} & {41.89$\pm$0.11 } & {36.23$\pm$0.60} & {36.26$\pm$0.63} & {36.59$\pm$0.27} & {24.33$\pm$0.01} & {46.18$\pm$0.08} & \textbf{48.97$\pm$0.83}\\

 \cmidrule(lr{0em}){2-12}

& \multirow{1}{*}{ {NIID}} & {13.14$\pm$5.02} & {18.46$\pm$0.83} & {12.98$\pm$5.00} & {34.27$\pm$0.04} & {10.73$\pm$0.01} & {10.71$\pm$0.01} & {10.72$\pm$0.01 } & {10.05$\pm$0.00} & {30.32$\pm$1.43} & \textbf{38.27$\pm$1.45}\\


\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\begin{tablenotes}
    \scriptsize 
     \item[1] We select the best result in the first 18 and 6 communication rounds for the training on MNIST and CIFAR-10, respectively.
     \item[2] Each client contributes 1 distilled image per class (Img/Cls = 1) from its local dataset. 
   \end{tablenotes}
\end{threeparttable}
\end{table*}
